On the Value of Oversampling for Deep Learning in Software Defect Prediction

One truism of deep learning is that the automatic feature engineering (seen in the first layers of those networks) excuses data scientists from performing tedious manual feature engineering prior to running DL. For the specific case of deep learning for defect prediction, we show that that truism is false. Specifically, when we preprocess data with a novel oversampling technique called fuzzy sampling, as part of a larger pipeline called GHOST (Goal-oriented Hyper-parameter Optimization for Scalable Training), then we can do significantly better than the prior DL state of the art in 14/20 defect data sets. Our approach yields state-of-the-art results significantly faster deep learners. These results present a cogent case for the use of oversampling prior to applying deep learning on software defect prediction datasets.

==> encoded_results.tex <==
\newcommand{\green}[1]{\cellcolor{green!20}\textcolor{black}{#1}}
\newcommand{\red}[1]{\cellcolor{red!20}\textcolor{black}{#1}}

\begin{table}[!t]
\caption{Encoded results.
Cells show medians of 20 runs.
 \colorbox{green!20}{ Green} shows  results that have improved with the encoded output, \colorbox{red!20}{red} shows results that have worsened. White cells show ties. All comparisons are made using a Scott-Knott test, as described in \S \ref{sec:stats}.
}\scriptsize
\label{tab:encoded-results}
\centering {\scriptsize
\begin{tabular}{ll|llll}
\toprule
&       & AUC  & popt20 & recall & pf  \\ \midrule
\multirow{3}{*}{ivy}	& DL & \red{0.53} & \green{0.53} & \red{0.11} & \green{0.04} \\
	& DODGE & \green{0.73} & \green{0.54} & \red{0.82} & 0.37 \\
	& GHOST & \green{0.73} & \green{0.60} & \red{0.82} & \green{0.35} \\ \midrule
\multirow{3}{*}{lucene}	& DL & \green{0.61} & \green{0.85} & \red{0.65} & \green{0.38} \\
	& DODGE & 0.6 & \red{0.61} & \red{0.64} & \red{0.44} \\
	& GHOST & \green{0.6} & \red{0.68} & \red{0.66} & \red{0.46} \\ \midrule
\multirow{3}{*}{poi}	& DL & \red{0.55} & \green{0.82} & \red{0.14} & \green{0.05} \\
	& DODGE & \red{0.71} & \red{0.61} & \red{0.58} & \green{0.15} \\
	& GHOST & \red{0.63} & 0.72 & \red{0.62} & 0.35 \\ \midrule
\multirow{3}{*}{synapse}	& DL & \red{0.53} & \green{0.59} & \red{0.08} & \green{0.02} \\
	& DODGE & \red{0.58} & \green{0.58} & \red{0.28} & \green{0.14} \\
	& GHOST & \green{0.69} & \green{0.63} & \red{0.58} & \green{0.2} \\ \midrule
\multirow{3}{*}{velocity}	& DL & \red{0.48} & \green{0.68} & \green{0.95} & \red{1.0} \\
	& DODGE & \red{0.59} & \red{0.63} & 0.75 & \red{0.57} \\
	& GHOST & \red{0.56} & \red{0.58} & \red{0.65} & \red{0.54} \\ \midrule
\multirow{3}{*}{camel}	& DL & 0.54 & \green{0.59} & 0.09 & \green{0.02} \\
	& DODGE & \red{0.56} & \red{0.29} & \red{0.26} & \green{0.13} \\
	& GHOST & \red{0.57} & \red{0.43} & \red{0.51} & \green{0.34} \\ \midrule
\multirow{3}{*}{jedit}	& DL & \green{0.65} & \green{0.60} & 0.45 & 0.11 \\
	& DODGE & \green{0.69} & \green{0.73} & \green{0.64} & \green{0.22}  \\
	& GHOST & \red{0.62} & \green{0.54} & 0.64 & 0.39 \\ \midrule
\multirow{3}{*}{log4j}	& DL & \red{0.56} & \green{1.0} & \red{0.27} & 0.12 \\
	& DODGE & \green{0.63} & \red{0.65} & \red{0.34} & \green{0.06} \\
	& GHOST & \red{0.59} & \red{0.66} & \red{0.42} & \red{0.25} \\ \midrule
\multirow{3}{*}{xalan}	& DL & 0.6 & \green{1.0} & 0.21 & \green{0.0} \\
	& DODGE & \red{0.67} & \red{0.52} & \red{0.35} & \green{0.0} \\
	& GHOST & \red{0.73} & \red{0.61} & \red{0.55} & \green{0.09} \\ \midrule
\multirow{3}{*}{xerces}	& DL & 0.52 & \green{0.95} & 0.03 & 0.0 \\
	& DODGE & \red{0.54} & \red{0.56} & \red{0.16} & \green{0.07} \\
	& GHOST & \red{0.58} & \green{0.61} & \red{0.48} & \green{0.34} \\
                                         \bottomrule
\end{tabular} }
\end{table}
